CoReEcho: Continuous Representation Learning for 2D+time Echocardiography Analysis

Deep learning (DL) models have been advancing automatic medical image analysis on various modalities, including echocardiography, by offering a comprehensive end-to-end training pipeline. This approach enables DL models to regress ejection fraction (EF) directly from 2D+time echocardiograms, resulting in superior performance. However, the end-to-end training pipeline makes the learned representations less explainable. The representations may also fail to capture the continuous relation among echocardiogram clips, indicating the existence of spurious correlations, which can negatively affect the generalization. To mitigate this issue, we propose CoReEcho, a novel training framework emphasizing continuous representations tailored for direct EF regression. Our extensive experiments demonstrate that CoReEcho: 1) outperforms the current state-of-the-art (SOTA) on the largest echocardiography dataset (EchoNet-Dynamic) with MAE of 3.90 & R2 of 82.44, and 2) provides robust and generalizable features that transfer more effectively in related downstream tasks. The code is publicly available at https://github.com/fadamsyah/CoReEcho.

==> algorithm.tex <==
\begin{algorithm}[!t]

    \centering

    \caption{Volumetric Adversarial Frequency Attack (\textbf{VAFA}) }\label{alg:afa-algo}

    \footnotesize

    \begin{algorithmic}[1]

        \State Number of Steps: $T$,~~Quantization Threshold: $ q_{\text{max}}$

        % \State \textbf{Input:} $\mathrm{X},\mathrm{Y}$~~~~\textbf{Output:} $\mathrm{X}^{\prime}$ 

        \State \textbf{Input:} $\mathrm{X}\in\mathbb{R}^{H\times W\times D},\mathrm{Y}\in\{0,1\}^{\mathrm{NumClass}\times H\times W\times D}~~~~\textbf{Output:~} \mathrm{X}^{\prime}\in\mathbb{R}^{H\times W\times D}$ 

        % \Statex

        \Function{{\textbf{VAFA}}}{X,Y}

             % \State $\bm{\mathrm{q}}_i \gets \bm{1}$ \Comment{Initialize all \textit{quantization tables} with ones.~~~~}

             \State $\bm{\mathrm{q}}_i \gets \bm{1}~~~~~\forall~i\in\{1,2,\dots,n\}$ \Comment{Initialize all \textit{quantization tables} with ones.~~~~}

             \For{$t \gets 1$ to $T$}

                 \State $ \{\bm{\mathrm{x}}_i\}_{i=1}^{n} \gets \text{Split}(\mathrm{X})$~\Comment{Split $\mathrm{X}$ into 3D patches of size $(h\times w \times d)~~$}

                 % \State \Comment{Drop information in frequency-domain}

                 \State $\bm{\mathrm{x}}_i^{\prime} \gets \mathcal{D}_{I}\big(~\varphi\bm{(}\mathcal{D}(\bm{\mathrm{x}}_i),\bm{\mathrm{q}}_{i}\bm{)}~\big)~~~\forall~i\in\{1,2,\dots,n\}$ \Comment{Frequency Perturbation~~~}

                 \State $ \mathrm{X}^{\prime} \gets \text{Merge}(\{\bm{\mathrm{x}}_i^{\prime}\}_{i=1}^{n})$~\Comment{Merge all adversarial patches to form $\mathrm{X}^{\prime}~~~~~$}

                 \State $\mathcal{L}( {\mathrm{X}}, {\mathrm{X}}^{\prime}, {\mathrm{Y}} ) = \mathcal{L}_{\mathrm{dice}} (\mathcal{M}_{\theta}({\mathrm{X}}^{\prime}), {\mathrm{Y}}) - \mathcal{L}_{\mathrm{ssim}}({\mathrm{X}},{\mathrm{X}}^{\prime})$

                 \State $\bm{\mathrm{q}}_{i} \gets \bm{\mathrm{q}}_{i} +~\mathrm{sign}(\nabla_{\bm{\mathrm{q}}_{i}} \mathcal{L}) ~~~~~\forall~i\in\{1,2,\dots,n\}$

                 \State $\bm{\mathrm{q}}_{i} \gets \mathrm{clip}(\bm{\mathrm{q}}_{i},~ \text{min=1},~\text{max=}q_{\text{max}})~~~~~\forall~i\in\{1,2,\dots,n\}$

             \EndFor

        \EndFunction

        \State \textbf{Return}  $\mathrm{X}^{\prime}$

    \end{algorithmic}

\end{algorithm}

\begin{algorithm}[!t]

    \centering

    \caption{Volumetric Adversarial Frequency Training (\textbf{VAFT})}\label{alg:afa-at}

    \footnotesize

    \begin{algorithmic}[1]

        \State Train Dataset: $\mathcal{X}=\{({\mathrm{X}}_i,{\mathrm{Y}}_i)\}_{i=1}^{N}$,~~${\mathrm{X}}_i \in \mathbb{R}^{H\times W\times D}$,~~${\mathrm{Y}}_i \in \{0,1\}^{\mathrm{NumClass}\times H\times W\times D}$

        \State NumSamples=$N$, BatchSize=$B$, Target Model: $\mathcal{M}_{\theta}$,~AT Robust Model: $\mathcal{M}_{_{\text{\faShield*}}}$

        % \State Clean Logits: $\bm{\mathrm{z}} \gets \mathcal{M}_{\theta}({\mathrm{X}})$,~Adversarial Logits: $\bm{\mathrm{z}}^{\prime} \gets \mathcal{M}_{\theta}({\mathrm{X}}^{\prime})$

        % \Statex

        \For{$i\gets 1~\text{to}~ \text{NumEpochs}$}

        \For{$j\gets 1~\text{to}~ \lfloor{N/B}\rfloor$}

        \State Sample a mini-batch $\mathcal{B} \subseteq \mathcal{X}$ of size $B$

        \State ${\mathrm{X}}^{\prime} \gets \textbf{VAFA}({\mathrm{X}},{\mathrm{Y}})~~\forall ({\mathrm{X}},{\mathrm{Y}})\in\mathcal{B}$ \Comment{Adv. Freq. Attack on clean images.}

        % \State $\bm{\mathrm{z}} \gets \mathcal{M}_{\theta}({\mathrm{X}})$,~~~~~ $\bm{\mathrm{z}}^{\prime} \gets \mathcal{M}_{\theta}({\mathrm{X}}^{\prime})$

        % \State $\mathcal{L}_{\mathrm{fr}}({\mathrm{X}},{\mathrm{X}^{\prime}}) \gets \|\mathcal{D}(\bm{\mathrm{z}})-\mathcal{D}(\bm{\mathrm{z}}^{\prime})\|_1$ 

        \State $\mathcal{L} = \mathcal{L}_{\text{dice}} (\mathcal{M}_{\theta}({\mathrm{X}}), {\mathrm{Y}})+ \mathcal{L}_{\mathrm{dice}}(\mathcal{M}_{\theta}({\mathrm{X}^{\prime}}),{\mathrm{Y}})+ \mathcal{L}_{\mathrm{fr}}(\mathcal{M}_{\theta}({\mathrm{X}}),\mathcal{M}_{\theta}({\mathrm{X}}^{\prime}))$

        \State Backward pass and update $\mathcal{M}_{\theta}$

        \EndFor

        \EndFor

        \State  $\mathcal{M}_{\Scale[0.4]{{{\text{\faShield*}}}}} \gets \mathcal{M}_{\theta}$ \Comment{AT robust model after training completion.}

        \State \textbf{Return} $\mathcal{M}_{_{{\text{\faShield*}}}}$

    \end{algorithmic}

\end{algorithm}
